The GENEA Challenge 2023: A large scale evaluation of gesture generation models in monadic and dyadic settings

This paper reports on the GENEA Challenge 2023, in which participating teams built speech-driven gesture-generation systems using the same speech and motion dataset, followed by a joint evaluation. This year's challenge provided data on both sides of a dyadic interaction, allowing teams to generate full-body motion for an agent given its speech (text and audio) and the speech and motion of the interlocutor. We evaluated 12 submissions and 2 baselines together with held-out motion-capture data in several large-scale user studies. The studies focused on three aspects: 1) the human-likeness of the motion, 2) the appropriateness of the motion for the agent's own speech whilst controlling for the human-likeness of the motion, and 3) the appropriateness of the motion for the behaviour of the interlocutor in the interaction, using a setup that controls for both the human-likeness of the motion and the agent's own speech. We found a large span in human-likeness between challenge submissions, with a few systems rated close to human mocap. Appropriateness seems far from being solved, with most submissions performing in a narrow range slightly above chance, far behind natural motion. The effect of the interlocutor is even more subtle, with submitted systems at best performing barely above chance. Interestingly, a dyadic system being highly appropriate for agent speech does not necessarily imply high appropriateness for the interlocutor. Additional material is available via the project website at https://svito-zar.github.io/GENEAchallenge2023/ .

==> tables/human-likeness_table.tex <==
\iffalse
\begin{table}[!t]
\centering%
\caption{Summary statistics of user-study ratings from the human-likeness study, with confidence intervals at the level $\alpha=0.05$. Conditions are ordered by decreasing sample median rating.}
\label{tab:humlikestats}
\begin{tabular}{@{}l|cc@{}}
\toprule
Condi- & \multicolumn{2}{c@{}}{Human-likeness} \\
tion & Median & Mean\\
\midrule
NA & $71\in{}[70,\,71]$ & $68.4{\pm}1.0$\\
SG & $69\in{}[67,\,70]$ & $65.6{\pm}1.4$\\
SF & $65\in{}[64,\,67]$ & $63.6{\pm}1.3$\\
SJ & $51\in{}[50,\,53]$ & $51.8{\pm}1.3$\\
SL & $51\in{}[50,\,51]$ & $50.6{\pm}1.3$\\
SE & $50\in{}[49,\,51]$ & $50.9{\pm}1.3$\\
SH & $46\in{}[44,\,49]$ & $45.1{\pm}1.5$\\
BD & $46\in{}[43,\,47]$ & $45.3{\pm}1.4$\\
SD & $45\in{}[43,\,47]$ & $44.7{\pm}1.3$\\
BM & $43\in{}[42,\,45]$ & $42.9{\pm}1.3$\\
SI & $40\in{}[39,\,43]$ & $41.4{\pm}1.4$\\
SK & $37\in{}[35,\,40]$ & $40.2{\pm}1.5$\\
SA & $30\in{}[29,\,31]$ & $32.0{\pm}1.3$\\
SB & $24\in{}[23,\,27]$ & $27.4{\pm}1.3$\\
SC & $\hphantom{0}9\in{}[\hphantom{0}9,\,\hphantom{0}9]$ & $11.6{\pm}0.9$\\
\bottomrule
\end{tabular}
\end{table}
\fi 
\begin{table}[!t]
    \centering%
    \caption{Summary statistics of user-study ratings from the human-likeness study, with confidence intervals at the level $\alpha=0.05$. Conditions are ordered by decreasing sample median rating.}
    \label{tab:append_humlikestats}
    \begin{tabular}{@{}lcc|lcc@{}}
    \toprule
    Condi- & \multicolumn{2}{c|@{}}{Human-likeness} & Condi- & \multicolumn{2}{c@{}}{Human-likeness} \\
    tion & Median & Mean & tion & Median & Mean\\
    \midrule
    NA & $71\in{}[70,\,71]$ & $68.4{\pm}1.0$ & SD & $45\in{}[43,\,47]$ & $44.7{\pm}1.3$\\
    SG & $69\in{}[67,\,70]$ & $65.6{\pm}1.4$ & BM & $43\in{}[42,\,45]$ & $42.9{\pm}1.3$\\
    SF & $65\in{}[64,\,67]$ & $63.6{\pm}1.3$ & SI & $40\in{}[39,\,43]$ & $41.4{\pm}1.4$\\
    SJ & $51\in{}[50,\,53]$ & $51.8{\pm}1.3$ & SK & $37\in{}[35,\,40]$ & $40.2{\pm}1.5$\\
    SL & $51\in{}[50,\,51]$ & $50.6{\pm}1.3$ & SA & $30\in{}[29,\,31]$ & $32.0{\pm}1.3$\\
    SE & $50\in{}[49,\,51]$ & $50.9{\pm}1.3$ & SB & $24\in{}[23,\,27]$ & $27.4{\pm}1.3$\\
    SH & $46\in{}[44,\,49]$ & $45.1{\pm}1.5$ & SC & $\hphantom{0}9\in{}[\hphantom{0}9,\,\hphantom{0}9]$ & $11.6{\pm}0.9$\\
    BD & $46\in{}[43,\,47]$ & $45.3{\pm}1.4$ & & \\
    \bottomrule
\end{tabular}
\end{table}

==> tables/response_data_table.tex <==
\begin{table*}[]
    \centering
    \caption{Statistics of user-study participants included in the statistical analyses.}\label{tab:users}
    \begin{tabular}{@{}lccccccc@{}}
    \toprule
    \multirow{2}{*}{Study} & Number of & \multicolumn{2}{c}{Videos watched} & \multicolumn{2}{c}{Ratings per condition} & Median time & Median pay\\
    \cmidrule{3-6}
    & test takers & per page & per test taker & min & max & taken& (in GBP/hour)\\
    \midrule
    Human-likeness & 200 & 8 & 80 & \hphantom{0}938 & 2000 & 25.3 min & 14.25\\
    Speech approp. & 600 & 2 & 80 & 1766&1815& 23.8 min& 15.10\\
    Interloc. approp. & 423 & 2 & 80 & \hphantom{0}993 & 1019 & 30.3 min & 11.86\\  
    \bottomrule
    \end{tabular}
\end{table*}
